A Practitioner's Guide to MDP Model Checking Algorithms

Model checking undiscounted reachability and expected-reward properties on Markov decision processes (MDPs) is key for the verification of systems that act under uncertainty. Popular algorithms are policy iteration and variants of value iteration; in tool competitions, most participants rely on the latter. These algorithms generally need worst-case exponential time. However the problem can equally be formulated as a linear program, solvable in polynomial time. In this paper, we give a detailed overview of today's state-of-the-art algorithms for MDP model checking with a focus on performance and correctness. We highlight their fundamental differences, and describe various optimisations and implementation variants. We experimentally compare floating-point and exact-arithmetic implementations of all algorithms on three benchmark sets using two probabilistic model checkers. Our results show that (optimistic) value iteration is a sensible default, but other algorithms are preferable in specific settings. This paper thereby provides a guide for MDP verification practitioners -- tool builders and users alike.

==> 6_challenging.tex <==
\section{Challenging Models}

\color{red}
I took the following quote from~\cite[Sect. 6]{DBLP:conf/cav/JungesTS20} 
`we observe that OVI is typically the fastest, but EPI does not suffer from the numerical worst-cases as OVI does. If an observation trace is unlikely, the unrolled MDP constitutes a numerically challenging problem, in particular for value-iteration based model checkers.`
\color{black}

Haddad-Monmege (made into a non-trivial MDP), numerically hard (Sebastian), QVBS (some Markov automata, Tim)

\color{red}
The following link contains a worst-case setting for policy iteration. I dont know whether it is clear that this is good for value iteration...
https://arxiv.org/pdf/1003.3418.pdf
\color{black}

How we selected challenging models from QComp: 
either unguaranteed VI time > model construction time (i.e. non-trivial, more time to solve a state than to construct it) 
or VI returns wrong result.


%The following is just a collection of things I don't want to forget. Needs to be polished etc.
It is surprisingly hard to find Markov decision processes that are hard for value iteration. 
In~\cite{KRSW22}, the authors found several SGs that were difficult for VI. In particular, using PI for the SG and then LP for the MDP was better than VI.
However, extracting those MDPs showed that they are all easy for VI.
Similarly, [Maxi-ATVA-to-appear] used a random generation of SGs, many of which were challenging for the solutions algorithms, even though the state space size was limited to 10,000.
When using the same random generation for MDPs, all models were solved in seconds. Even scaling up the models to the point where building them took 20 minutes and reducing the occurring transition probabilities did not yield a challenging model.
This is in contrast to what \url{https://www.sciencedirect.com/science/article/abs/pii/S0360835215002545} found: their random generation returned models where LP beat PI. 
However, they consider \textit{discounted} reward and they don't describe their random generation precisely enough such that one could expect to reproduce their results. 


==> q_plots.tex <==
\section*{Further Plots}
{\color{red} TQ: This is a playground for creating plots}


% Available tool.config identifiers with number of qvbs benchmarks they solve
%	Storm.vi2pi-gmres: 407
%	Storm.vi2pi-vi: 399
%	Storm.vi2pi-lu: 290
%	Storm.vi2pi-ovi: 273
%	Storm.vi2pi-exactlu: 400
%	Storm.vi2pi-mecq-topo-gmres: 411
%	Storm.vi2pi-mecq-topo-vi: 381
%	Storm.vi2pi-mecq-topo-ovi: 292
%	Storm.vi2pi-mecq-topo-lu: 326
%	Storm.vi2pi-mecq-topo-exactlu: 348
%	Storm.vi: 428
%	Storm.vi-topo: 427
%	Storm.vi-mecq: 428
%	Storm.vi-mecq-topo: 427
%	Storm.ovi-topo: 435
%	Storm.ovi: 435
%	Storm.pi-vi: 397
%	Storm.pi-ovi: 272
%	Storm.pi-lu: 290
%	Storm.pi-exactlu: 371
%	Storm.pi-mecq: 398
%	Storm.pi-mecq-topo-lu: 324
%	Storm.pi: 399
%	Storm.pi-mecq-topo-vi: 375
%	Storm.pi-mecq-topo-exactlu: 333
%	Storm.pi-mecq-topo-ovi: 287
%	Storm.pi-topo: 402
%	Storm.pi-mecq-topo: 402
%	Storm.lp-mecq-topo-soplex-exact: 367
%	Storm.lp: 399
%	Storm.lp-mecq-topo-gurobi-4autoinit: 370
%	Storm.lp-gurobi-4autoiniteq: 380
%	Storm.lp-mecq-topo-glpk: 359
%	Storm.lp-nobnds: 400
%	Storm.lp-gurobi-4dualsimplnobnds: 399
%	Storm.lp-mecq-topo-z3-exact: 306
%	Storm.lp-soplex-nobnds: 295
%	Storm.lp-mecq: 399
%	Storm.lp-gurobi-4autoeq: 389
%	Storm.lp-mecq-topo-gurobi-4primalsimpl: 399
%	Storm.lp-mecq-topo-gurobi-4autoeq: 370
%	Storm.lp-mecq-topo-gurobi-4autonobnds: 369
%	Storm.lp-gurobi-4autonobnds: 397
%	Storm.lp-mecq-topo-gurobi-16auto: 415
%	Storm.lp-gurobi-16autonobnds: 397
%	Storm.lp-gurobi-4auto: 397
%	Storm.lp-topo: 411
%	Storm.lp-gurobi-4barriernobnds: 398
%	Storm.lp-mecq-topo-gurobi-4autoiniteq: 376
%	Storm.lp-mecq-topo-gurobi-4auto: 414
%	Storm.lp-soplex-exactnobnds: 287
%	Storm.lp-gurobi-4primalsimplnobnds: 385
%	Storm.lp-gurobi-4autoinit: 396
%	Storm.lp-mecq-topo-gurobi-4dualsimpl: 411
%	Storm.lp-mecq-topo-gurobi-4barrier: 412
%	Storm.lp-mecq-topo-soplex: 388
%	Storm.lp-z3-exactnobnds: 217
%	Storm.lp-glpk-nobnds: 268
%	Storm.lp-mecq-topo: 411
%	Storm.rs-exact: 240
%	Storm.rs-mecq-topo-exact: 340
%	Storm.best: 436



% Available benchmark sets
% qvbs-full (currently 489 benchmarks after dropping all where storm builds >= 15 minutes)
% qvbs-hard (currently 31 benchmarks after dropping all from qvbs-full that are either checked in <= 1sec or where storm.vi is faster than model building)
% premise (200 benchmarks from the premise case studies)


\subsection*{Quantile Plots}
% Arguments:
% #1: csv filename
% #2: comma separated list of tool.config/color items}
% #3: comma separated list of readable config names 
% #4: xmin
% #5: xmax
% #6: ymin
% #7: ymax
\begin{figure}[t]
\centering
\begin{subfigure}{0.5\textwidth}%
\quantileplot{plotdata/quantile-qvbs-full.csv}
{Storm.vi/color1, Storm.pi/color2, Storm.lp/color3, Storm.vi-mecq-topo/color4, Storm.pi-mecq-topo/color5, Storm.lp-mecq-topo/color6}
{VI, PI, LP, VI-topo, PI-topo, LP-topo}
{0}{\numqvbsfull}{0.1}{1800}
\caption{Approximate}
\label{fig:plot:storm:approx}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
\quantileplot{plotdata/quantile-qvbs-full.csv}
{Storm.rs-mecq-topo-exact/color1, Storm.pi-mecq-topo-exactlu/color2, Storm.vi2pi-mecq-topo-exactlu/color3, Storm.lp-mecq-topo-soplex-exact/color4, Storm.lp-mecq-topo-z3-exact/color5}
{RS, PI, PI-warm, LP-sopl, LP-z3}
{0}{\numqvbsfull}{0.1}{1800}
\caption{Exact (all topo)}
\label{fig:plot:storm:exact}
\end{subfigure}
\caption{Comparison of methods in Storm}
\label{fig:plot:storm}
\end{figure}



\begin{figure}[t]
\centering
\begin{subfigure}{0.5\textwidth}%
\quantileplot{plotdata/quantile-qvbs-full.csv}
{Storm.vi/color1, Storm.lp-glpk-nobnds/color2, Storm.lp-nobnds/color3, Storm.lp-soplex-nobnds/color4, Storm.lp-z3-exactnobnds/color5}
{(VI), glpk, gurobi, soplex, z3}
{0}{\numqvbsfull}{0.1}{1800}
\caption{Storm}
\label{fig:plotexact:a}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
\quantileplot{plotdata-mcsta/quantile-qvbs-full.csv}
{mcsta.vi/color1, mcsta.lp-copt-mono/color2, mcsta.lp-cplex-mono/color3, mcsta.lp-glop-mono/color4, mcsta.lp-gurobi-mono/color5, mcsta.lp-highs-mono/color6, mcsta.lp-lpsolve-mono/color7, mcsta.lp-mosek-mono/color8}
{(VI), copt, cplex, glop, gurobi, highs, lpsolve, mosek}
{0}{\numqvbsfull}{0.1}{1800}
\caption{mcsta}
\label{fig:plotexact:b}
\end{subfigure}
\caption{Comparison of LP solvers in Storm and mcsta}
\end{figure}

\begin{figure}[t]
\centering
\begin{subfigure}{0.5\textwidth}%
\quantileplot{plotdata/quantile-qvbs-full.csv}
{Storm.lp-gurobi-4autonobnds/color1, Storm.lp-gurobi-4primalsimplnobnds/color2, Storm.lp-gurobi-4dualsimplnobnds/color3, Storm.lp-gurobi-4barriernobnds/color4}
{auto, prim, dual, barrier}
{0}{\numqvbsfull}{0.1}{1800}
\caption{Gurobi, using 4 threads}
\label{fig:plotexact:a}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
\quantileplot{plotdata/quantile-qvbs-full.csv}
{Storm.lp-nobnds/color1, Storm.lp-gurobi-4autonobnds/color2, Storm.lp-gurobi-16autonobnds/color3}
{1, 4, 16}
{0}{\numqvbsfull}{0.1}{1800}\caption{Gurobi, using auto}
\label{fig:plotexact:b}
\end{subfigure}
\caption{Comparison of Gurobi methods in Storm}
\end{figure}

\begin{figure}[t]
\centering
\begin{subfigure}{0.5\textwidth}%
\quantileplot{plotdata/quantile-qvbs-full.csv}
{Storm.lp-gurobi-4autonobnds/color1, Storm.lp-gurobi-4auto/color2, Storm.lp-gurobi-4autoinit/color3, Storm.lp-gurobi-4autoeq/color4, Storm.lp-gurobi-4autoiniteq/color5}
{default, bnds, init+bnds, eq+bnds, init+eq+bnds}
{0}{\numqvbsfull}{0.1}{1800}
\caption{monolithic}
\label{fig:plotexact:a}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
\quantileplot{plotdata/quantile-qvbs-full.csv}
{Storm.lp-mecq-topo-gurobi-4autonobnds/color1, Storm.lp-mecq-topo-gurobi-4auto/color2, Storm.lp-mecq-topo-gurobi-4autoinit/color3, Storm.lp-mecq-topo-gurobi-4autoeq/color4, Storm.lp-mecq-topo-gurobi-4autoiniteq/color5}
{default, bnds, init+bnds, eq+bnds, init+eq+bnds}
{0}{\numqvbsfull}{0.1}{1800}\caption{topological}
\label{fig:plotexact:b}
\end{subfigure}
\caption{Comparison of Gurobi methods in Storm  using 4 threads and auto}
\end{figure}

\begin{figure}[t]
\centering
\begin{subfigure}{0.5\textwidth}%
\quantileplot{plotdata/quantile-qvbs-full.csv}
{Storm.lp-nobnds/color5, Storm.vi2lp-gurobi-nobnds/color2, Storm.lp-soplex-exactnobnds/color3, Storm.vi2lp-soplex-exactnobnds/color4, Storm.vi/color1}
{gurobi-cold, gurobi-warm, soplex-cold, soplex-warm, VI}
{0}{\numqvbsfull}{0.1}{1800}
\caption{lp}
\label{fig:plotexact:a}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}%
\quantileplot{plotdata/quantile-qvbs-full.csv}
{Storm.lp-mecq-topo/color5, Storm.vi2lp-mecq-topo-gurobi/color2, Storm.lp-mecq-topo-soplex-exact/color3, Storm.vi2lp-mecq-topo-soplex-exact/color4, Storm.vi-mecq-topo/color1}
{gurobi-cold, gurobi-warm, soplex-cold, soplex-warm, VI}
{0}{\numqvbsfull}{0.1}{1800}
\caption{lp-topo}
\label{fig:plotexact:a}
\end{subfigure}%
\caption{Effect of LP warm-starts}
\end{figure}


\begin{figure}[t]
\centering
\begin{subfigure}{0.5\textwidth}%
\quantileplot{plotdata/quantile-qvbs-full.csv}
{Storm.pi/color1, Storm.pi-vi/color2, Storm.pi-ovi/color3, Storm.pi-lu/color4, Storm.pi-exactlu/color5, Storm.vi2pi-gmres/color6, Storm.vi2pi-exactlu/color7}
{gmres, vi, ovi, lu, luexact, warm-gmres, warm-luex}
{0}{\numqvbsfull}{0.1}{1800}
\caption{monolithic}
\label{fig:plotexact:a}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
\quantileplot{plotdata/quantile-qvbs-full.csv}
{Storm.pi-mecq-topo/color1, Storm.pi-mecq-topo-vi/color2, Storm.pi-mecq-topo-ovi/color3, Storm.pi-mecq-topo-lu/color4, Storm.pi-mecq-topo-exactlu/color5, Storm.vi2pi-mecq-topo-gmres/color6, Storm.vi2pi-mecq-topo-exactlu/color7}
{gmres, vi, ovi, lu, luexact, warm-gmres, warm-luex}
{0}{\numqvbsfull}{0.1}{1800}
\caption{topological}
\label{fig:plotexact:b}
\end{subfigure}
\caption{Comparison of PI variants in Storm}
\end{figure}


\scatterplot{plotdata/scatter-qvbs-full.csv}{Storm.lp}{Gurobi Cold}{Storm.vi2lp-gurobi-nobnds}{Gurobi Warm}{false}%
\scatterplot{plotdata/scatter-qvbs-full.csv}{Storm.lp-soplex-exactnobnds}{Soplex Cold}{Storm.vi2lp-soplex-exactnobnds}{Soplex Warm}{false}



\iffalse

mcsta\\
\quantileplot{plotdata-mcsta/quantile-qvbs-full.csv}
{mcsta.vi/color1, mcsta.lp-copt-mono/color2, mcsta.lp-cplex-mono/color3, mcsta.lp-glop-mono/color4, mcsta.lp-gurobi-mono/color5, mcsta.lp-highs-mono/color6, mcsta.lp-lpsolve-mono/color7, mcsta.lp-mosek-mono/color8}
{VI, COPT, CPLEX, GLOP, GUROBI, HIGHS, LPSOLVE, MOSEK}
{0}{450}{0.1}{1800}
}%

qvbs-full\\
\quantileplot{plotdata/quantile-qvbs-full.csv}
{Storm.vi-mecq-topo/color1, Storm.ovi-topo/color2, Storm.pi-mecq-topo/color3, Storm.lp-mecq-topo/color4}
{VI-ectopo, OVI-ectopo, PI-ectopo, LP-ectopo}
{300}{489}{0.1}{1800}
%
\quantileplot{plotdata/quantile-qvbs-full.csv}
{Storm.vi-mecq-topo/color1, Storm.vi-mecq/color2, Storm.vi-topo/color3, Storm.vi/color4}
{VI-ectopo, VI-ec, VI-topo, VI}
{300}{489}{0.1}{1800}

\quantileplot{plotdata/quantile-qvbs-full.csv}
{Storm.pi-mecq-topo/color1, Storm.pi-mecq/color2, Storm.pi-topo/color3, Storm.pi/color4}
{PI-ectopo, PI-ec, PI-topo, PI}
{300}{489}{0.1}{1800}
%
\quantileplot{plotdata/quantile-qvbs-full.csv}
{Storm.lp-mecq-topo/color1, Storm.lp-mecq/color2, Storm.lp-topo/color3, Storm.lp/color4}
{lp-ectopo, lp-ec, lp-topo, lp}
{300}{489}{0.1}{1800}

qvbs-hard (all with ectopo)\\
\quantileplot{plotdata/quantile-qvbs-hard.csv}
{Storm.vi-mecq-topo/color1, Storm.ovi-topo/color2, Storm.pi-mecq-topo/color3, Storm.lp-mecq-topo/color4}
{VI, OVI, PI, LP}
{0}{31}{0.1}{1800}


premise (all with ectopo)\\
\quantileplot{plotdata/quantile-premise.csv}
{Storm.vi-mecq-topo/color1, Storm.ovi-topo/color2, Storm.pi-mecq-topo/color3, Storm.lp-mecq-topo/color4}
{VI, OVI, PI, LP}
{0}{200}{0.1}{200}

\pagebreak
\subsection*{Scatter Plots}
% Arguments:
% #1: csv filename
% #2: tool.config identifier for x-axis
% #3: label for x-axis
% #4: tool.config identifier for y-axis
% #5: label for y-axis
% #6: trigger showing the legend (true/false)

qvbs-full
\scatterplot{plotdata/scatter-qvbs-full.csv}{Storm.vi-mecq-topo}{VI with mecq and topo}{Storm.pi-mecq-topo}{PI with mecq and topo}{false}
\scatterplot{plotdata/scatter-qvbs-full.csv}{Storm.vi-mecq-topo}{VI with mecq and topo}{Storm.lp-mecq-topo}{LP with mecq and topo}{false}

\scatterplot{plotdata/scatter-qvbs-full.csv}{Storm.pi-mecq-topo}{PI with mecq and topo}{Storm.lp-mecq-topo}{LP with mecq and topo}{false}
\scatterplot{plotdata/scatter-qvbs-full.csv}{Storm.pi-mecq-topo}{PI with mecq and topo}{Storm.pi-topo}{PI with topo}{false}
\pagebreak
qvbs-hard

\scatterplot{plotdata/scatter-qvbs-hard.csv}{Storm.vi-mecq-topo}{VI with mecq and topo}{Storm.pi-mecq-topo}{PI with mecq and topo}{false}
\scatterplot{plotdata/scatter-qvbs-hard.csv}{Storm.vi-mecq-topo}{VI with mecq and topo}{Storm.lp-mecq-topo}{LP with mecq and topo}{false}

\scatterplot{plotdata/scatter-qvbs-hard.csv}{Storm.pi-mecq-topo}{PI with mecq and topo}{Storm.lp-mecq-topo}{LP with mecq and topo}{false}
\scatterplot{plotdata/scatter-qvbs-hard.csv}{Storm.pi-mecq-topo}{PI with mecq and topo}{Storm.pi-topo}{PI with topo}{false}

\pagebreak
premise

\scatterplot{plotdata/scatter-premise.csv}{Storm.vi-mecq-topo}{VI with mecq and topo}{Storm.pi-mecq-topo}{PI with mecq and topo}{false}
\scatterplot{plotdata/scatter-premise.csv}{Storm.vi-mecq-topo}{VI with mecq and topo}{Storm.lp-mecq-topo}{LP with mecq and topo}{false}

\scatterplot{plotdata/scatter-premise.csv}{Storm.pi-mecq-topo}{PI with mecq and topo}{Storm.lp-mecq-topo}{LP with mecq and topo}{false}
\scatterplot{plotdata/scatter-premise.csv}{Storm.pi-mecq-topo}{PI with mecq and topo}{Storm.pi-topo}{PI with topo}{false}

\fi



